Measuring and Understanding Throughput of Network Topologies

High throughput is of particular interest in data center and HPC networks. Although myriad network topologies have been proposed, a broad head-to-head comparison across topologies and across traffic patterns is absent, and the right way to compare worst-case throughput performance is a subtle problem. In this paper, we develop a framework to benchmark the throughput of network topologies, using a two-pronged approach. First, we study performance on a variety of synthetic and experimentally-measured traffic matrices (TMs). Second, we show how to measure worst-case throughput by generating a near-worst-case TM for any given topology. We apply the framework to study the performance of these TMs in a wide range of network topologies, revealing insights into the performance of topologies with scaling, robustness of performance across TMs, and the effect of scattered workload placement. Our evaluation code is freely available.

==> artifact.tex <==

\section{Artifact Description: Measuring and Understanding Throughput of Network Topologies}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Abstract}
This artifact contains the code to generate the linear program (LP) for measuring throughput and the topologies used for evaluation. It also includes scripts to run the LP with the Gurobi LP solver and generate plots using gnuplot. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Description}
The LP generator takes as input a topology and a traffic type. In addition to the tested topologies, users can also specify their custom topologies which can be read from a file. Traffic types supported are all-to-all, random permutation and longest matching.

\subsubsection{Check-list (artifact meta information)}

{\small
\begin{itemize}
  \item {\bf Program: Java}
  \item {\bf Compilation:javac 1.7 or higher}
  \item {\bf Data set: Publicly available topologies included in the artifact}
  \item {\bf Run-time environment: Linux with LP solver (Gurobi/CPLEX) and gnuplot 4.4 or higher}
  \item {\bf Hardware: Any hardware}
  \item {\bf Experiment customization: Modify scripts to choose specific topology and traffic type }
  \item {\bf Publicly available?: Yes}
\end{itemize}
}

\subsubsection{How delivered}
Topobench is an open-source test bench released under the MIT license. The test bench and related instructions are hosted on Github. (https://github.com/ankitsingla/topobench)

\subsubsection{Hardware dependencies}
The test bench will run on any general purpose computer. However, the largest network that can be tested depends on available RAM and the topology being tested. This is due to the memory restrictions of the LP solvers. 

\subsubsection{Software dependencies}
Experiments in this paper were run on Ubuntu 14.04 with javac 1.8.0 and Gurobi 5.6. The scripts use gnuplot 4.4 or higher (for the pdfcairo terminal). But if you don't have it, you can still get the result files and plot them using other software.

\subsubsection{Datasets}
HPC and data center topologies evaluated in this paper are available in the folder \textit{lpmaker/graphs} and real-world graphs are available in the folder \textit{graphrepo}.

\subsection{Installation}
The test bench and instructions to use it can be downloaded from the Github repository - https://github.com/ankitsingla/topobench.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment workflow}
The experiments are run with shell scripts and the results are stored in text files.

Clone the test bench to local machine and compile:
\begin{lstlisting}
   $ git clone https://github.com/
       ankitsingla/topobench
   $ cd topobench
   $ javac lpmaker/ProduceLP.java
\end{lstlisting}

Run the scripts located in the folder \textit{scripts}:
\begin{lstlisting}
   $ bash scripts/fatCompare.sh
\end{lstlisting}

Plot using gnuplot scripts:
\begin{lstlisting}
   $ gnuplot gnuplotscripts/fatCompare.plt
\end{lstlisting}

%\begin{algorithm}[H]
%\begin{algorithmic}[1]
%\Statex{\$
%\end{algorithmic}
%\end{algorithm}
%\noindent{\setstretch{0.01}\rule{8cm}{0.4pt}}


Clean folders:
\begin{lstlisting}
   $ bash scripts/clean.sh
\end{lstlisting}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evaluation and expected result}

After running an experiment, the results are available in the folder \textit{resultfiles}. The results can be plotted using gnuplot (4.4+) using scripts in the folder \textit{gnuplotscripts}. The pdf plots are stored in the folder \textit{plots}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment customization}
Scripts can be modified to choose a specific topology and traffic matrix. The experiments were run with Gurobi 5.6 and gnuplot 4.6. However, any LP solver which can read the standard LP format (e.g., CPLEX) and any plotting software may be used.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Notes}

